Analyzing LLM Usage in an Advanced Computing Class in India

This study examines the use of large language models (LLMs) by undergraduate and graduate students for programming assignments in advanced computing classes. Unlike existing research, which primarily focuses on introductory classes and lacks in-depth analysis of actual student-LLM interactions, our work fills this gap. We conducted a comprehensive analysis involving 411 students from a Distributed Systems class at an Indian university, where they completed three programming assignments and shared their experiences through Google Form surveys. Our findings reveal that students leveraged LLMs for a variety of tasks, including code generation, debugging, conceptual inquiries, and test case creation. They employed a spectrum of prompting strategies, ranging from basic contextual prompts to advanced techniques like chain-of-thought prompting and iterative refinement. While students generally viewed LLMs as beneficial for enhancing productivity and learning, we noted a concerning trend of over-reliance, with many students submitting entire assignment descriptions to obtain complete solutions. Given the increasing use of LLMs in the software industry, our study highlights the need to update undergraduate curricula to include training on effective prompting strategies and to raise awareness about the benefits and potential drawbacks of LLM usage in academic settings.

==> files/04-evaluation.tex <==
We performed a three-layer thematic analysis\cite{braun_using_2006} on the qualitative data collected from the interviews and survey as explained in the methodology. This data was collated, merged, and finally categorized into three overarching themes - \textit{Usage Patterns and Benefits, Challenges, and Perceptions and Recommendations}. This enabled us to categorize and report our findings in a structured manner encompassing insights covering different aspects of the experience of using ChatGPT.
% \newcommand{\quotedtext}[1]{%
%    \noindent\textbf{\textit{{"#1"}}}%
% }

Table \ref{tab:interview_demographics} depicts the demographics of the participants of the interviews. The participants were taken from 8 different universities. Out of 17 participants, 8 were male and 9 were female. 6 participants were freshmen, 5 participants were sophomores, 2 participants were juniors, and 3 were seniors. This representation is influenced by the varying availability of students across different academic years owing to commitments such as internship drive preparations and placement preparations.
% \subsection{Emerging Usage Patterns and Benefits of using ChatGPT}
\subsection{Qualitative analysis of survey results}
\customheading{Usage Patterns adopted by Undergraduate Computer Science students.} Our findings show that the growing discussions and dialogue about ChatGPT was the starting point for most of our participants to try exploring this tool. Various participants talked about using it first just to discover its general and CS-specific capabilities. This was followed by trying it out for academic use cases such as assignments and take-home labs and eventually making regular use of it. Participants talked about trying it for writing codes or solving questions for their academic assignments to scope its capabilities. A participant mentioned that ChatGPT's conversational nature helped them to review and reinforce concepts and engage in discussions with it. A participant mentioned -

\quotedtext{\hlcyan{I've been using ChatGPT for about seven or eight months now. I heard about it from a fellow batchmate [...] when I was stuck on an assignment and then he recommended me to use ChatGPT for it. Initially, I used it rarely, but lately, it has become quite a handy tool.}} -[P14]

Participants talked about depending on ChatGPT for their \hlcyan{academic assignments and preparation for course tests and exams}. They mentioned that their usage would increase depending on the workload they had. Participants relied on ChatGPT when they had time constraints for assignments. They utilized it for tasks such as \hlcyan{information gathering, code generation, error identification, and more}. They broke down problems related to code and concepts, inputting them into ChatGPT while cross-checking outputs with their domain knowledge.

\quotedtext{\hlcyan{Earlier, when I would have to spend 2 hours to even find a basic approach for a problem, ChatGPT would give that to me in 2 minutes, and from there, I can build on that.}} -[P10]


A recurring usage pattern was observed: users sought answers from ChatGPT, cross-checked with peers or sources like Google Search, corrected errors with ChatGPT, and extracted accurate responses. \hlcyan{For code, they tested the generated code, sought error fixes from ChatGPT, and retrieved corrected versions}. Dependence on ChatGPT was observed to be very prominent, however, it has reduced as users started to recognize its current technical limitations and challenges. As a participant mentioned -


\quotedtext{\hlcyan{It significantly reduces the time I spend searching for solutions to
problems. It is like, you know, it points me in the right direction, and I can Google the rest up.}} -[P7]

\customheading{Emerging Benefits of using ChatGPT for Academic Tasks.} Our findings reveal ChatGPT's potential to support ideation among undergraduates. It is seen as a valuable tool for \hlcyan{initiating problem-solving} as it offers vast knowledge for \hlcyan{idea generation}. It was referred to as a comprehensive search engine that aids learning across various domains. The conversational aspect of it also eases onboarding and offers personalized insights. This helps with brainstorming and exploring unfamiliar CS domains. A participant mentioned -

\quotedtext{\hlcyan{It has become an indispensable tool that I rely on regularly to gather information,  brainstorm ideas, get the algorithm, and debug the code.}} -[P6]

While talking about use cases specific to computer science coursework, our participants talked about ChatGPT being a handy tool to quickly understand small details in \hlcyan{documentation and language semantics}. More so, ChatGPT could serve as an assistant to \hlcyan{debug coded algorithms} and learn more about them using its conversational nature. A participant mentioned how ChatGPT is better than other traditional online sources to assist in programming, such as Stack Overflow \cite{stack_overflow}, because one would need to recheck its generated answer using their own understanding and converse back and forth with ChatGPT, which cannot happen in other online resources where students directly copy-paste the answers they find.

\quotedtext{It is good for debugging the code someone has written because otherwise, people would anyway go to websites like Stack Overflow and follow things blindly, but using ChatGPT, they can at least know what they were doing wrong and where they could improve.} -[P12]

ChatGPT commonly came up as an effective learning assistant or a tutor. Participants talked about using it for \hlcyan{step-by-step explanations of questions, for example, programming questions,} which are not possible when referring to online resources for assistance in learning. More so, its conversational modality can aid in self-study sessions as you can ask it to explain \hlcyan{certain concepts in detail and ask follow-up questions}. ChatGPT is also being used to \hlcyan{generate practice questions on a topic}.

\quotedtext{For example, I was in a course, and the course did not have any pre-made content/questions. So, sir, asked ChatGPT to give us a bunch of questions for that course. And I think, though, that was kinda cool, and that is how it was used in a good way.} -[P12]

Participants mentioned that ChatGPT is great at \hlcyan{generating theoretical responses}. It's frequently used for \hlcyan{lengthy reports, projects, and assignment write-ups}. Some participants even used it for internship applications and resume content. Despite occasional inaccuracies, many considered it a valuable content-writing tool. A participant mentioned -

\quotedtext{I used it religiously for one of the humanities courses where we had to write a report. I wrote almost the entire thing with the help of ChatGPT. Other than that, I have used it to write some codes, get help in writing emails, etc.} -[P10]

\subsection{Thematic Analysis of Conversations of Students with LLMs}
\customheading{Usability and Reliability Challenges.} Through our interviews, we got a sense of the usability challenges that the participants face while using ChatGPT and how these factors affect their overall perception of ChatGPT and their usage behaviors around it. The process of accessing ChatGPT seemed to be a barrier to the effective use of the model. Participants reported that the process of signing into the website and the periodically repetitive nature of re-authenticating with their accounts hindered their smooth experience. A participant explained -

\quotedtext{It's not like quillbot\footnote{https://quillbot.com/}, you open it, do your work, and get out. I have to make a new account here, so it just encroaches on my brain - a new account.} -[P13]

ChatGPT did not seem very humanistic to some participants, and they felt like it was \textit{too programmed} to talk to naturally, especially when they require a specific answer. This was highlighted when participants mentioned that \hlcyan{ChatGPT felt repetitive in its answers for theoretical questions despite providing it with different prompts}. Many participants found using it to be out of their comfort zone, requiring explicit context-setting which was tedious. Some found it more time-consuming than a typical Google search, as they needed to \hlcyan{verify every answer it provided explicitly}.

\quotedtext{\hlcyan{One tedious task is to write prompts. If you have to tell something to a human, you say it in just one sentence, but here to get accurate results, you have to write it in four to five sentences to give prompts.}} -[P5]

When it comes to providing the proper prompts for ChatGPT, we found that participants were not satisfied with the responses they got for the \hlcyan{long, complex prompts} provided by them. This made them break down their prompts into smaller segments to extract \hlcyan{better results}, and in some cases, have to intervene on a line-to-line basis for their prompts. Writing well-structured prompts to get the right answer seemed like a challenge to many participants and meant that having the skill to set the right context before asking their question was a prerequisite to getting good quality results.

\quotedtext{\hlcyan{You have to double-check everything. You do it carefully, line by line, and make sure you exactly understand what it's doing. And most of the time, 80\% of the time, you'll have to edit it a lot to get it to work.}} -[P9]

Participants reported that ChatGPT does not meet their \hlcyan{academic and ideation requirements for course projects} as it fails to provide them with creative suggestions. Furthermore, participants found it to be \hlcyan{unreliable for programming}, as the more they used it for their \hlcyan{courses and debugging}, the more they reported encountering inaccuracies. Some participants highlighted the fact that ChatGPT \hlcyan{does not handle mathematical problems effectively}, causing them to rely on other sources for accurate answers. 

\quotedtext{\hlcyan{It tends to generate code snippets that might work but are not optimized or could be improved. In such cases, I have to manually refine the code. Also, there are times when it fails to understand complex questions properly, leading to irrelevant or inaccurate responses.}} -[P14] 

\customheading{Learning and Ethical Challenges.} Majority of the participants stated that they view ChatGPT in academics as a \textit{double-edged sword}. Participants appreciated ChatGPT as an assistant but suggested limiting its role to avoid making the human mind passive. Over-reliance could lead to \hlcyan{mental sluggishness and hinder effective learning and the cognitive thinking required to reach solutions to complex questions}. While useful for quick insights, participants noted its limitations in facilitating deep learning. One participant mentioned that it undermines rote learning, impacting their information retention.

\quotedtext{\hlcyan{It's helping as well, but at the same time, it's reducing human power and human thinking ability. Like we always depend on chat GPT for new ideas. We are not running our own minds.}} -[P5]

Some participants stated that they find the use of ChatGPT in academics unethical. They reported that using the tool for their academic tasks feels like an unethical shortcut, which leads to a feeling of guilt and is a blocker for human efforts and creativity.

\quotedtext{Sometimes I feel as though I am cheating by learning through it. I mean, sometimes, you know, it just feels wrong when it gets too easy?} -[P7]

% I asked ChatGPT what should be written in this section. ChatGPT's response is shared below. Please add all the relevant details as suggested by ChatGPT.

% \textcolor{red}{The evaluation section of a research paper presents the findings of the study and discusses the results in relation to the research objectives. In the context of the study on the actual usage of Large Language Models (LLMs) among computer science undergraduate students, the evaluation section should include the following key components:
% \begin{itemize}[leftmargin=*]
% \item \textbf{Presentation of Results:} Provide a comprehensive presentation of the survey and interview results. Include relevant statistics, charts, graphs, and qualitative excerpts to illustrate the findings effectively.
% \item \textbf{Analysis of Findings:} Interpret the results obtained from the survey responses and interview data. Discuss the patterns, trends, and key themes that emerged during the analysis. Compare and contrast the different responses from students to gain deeper insights.
% \item \textbf{Alignment with Research Objectives:} Evaluate how well the study's findings align with the research objectives and research questions stated in the introduction. Address whether the research objectives were adequately met, and discuss any unexpected or significant findings.
% \item \textbf{Discussion of Challenges and Opportunities:} Reflect on the challenges and opportunities associated with the actual usage of LLMs among students, as revealed in the survey and interview responses. Analyze the implications of these findings for both students and instructors.
% \item \textbf{Comparison with Prior Research:} Compare the current study's findings with those from previous research mentioned in the introduction. Highlight similarities, differences, or discrepancies and discuss potential reasons for any variations.
% \item \textbf{Generalizability of Findings:} Discuss the extent to which the study's findings can be generalized to other settings or contexts. Address any limitations that may impact the generalizability of the results.
% \item \textbf{Practical Implications:} Examine the practical implications of the study's findings for the computing education domain. Discuss how the insights gained can inform instructional practices, curriculum design, and the integration of LLMs in computer science courses.
% \item \textbf{Ethical Considerations:} Consider any ethical implications of the study's findings, particularly concerning student privacy, data protection, and the responsible use of LLMs in educational settings.
% \item \textbf{Recommendations for Future Research:} Offer suggestions for future research based on the study's outcomes. Identify areas that require further exploration and propose potential research directions to enhance the understanding of LLM usage in computing education.
% \item \textbf{Conclusion:} Summarize the key findings of the study and reiterate their significance in the context of the research objectives. Conclude with a closing statement that emphasizes the overall contribution of the research to the field of computing education.
% \end{itemize}
% }

\subsection{Perceptions and Recommendations}

Our findings indicate that conventional practices like Google search, textbooks, and peer assistance are favored over ChatGPT. Trust issues with ChatGPT's authenticity and personal comfort zone hesitations were observed. Some participants prioritized personal effort for practices like coding and gathering information themselves, deterring their interest in using ChatGPT as an academic aid. A participant mentioned ChatGPT's limitations compared to human creativity and efficiency, affecting their reliance on it.

\quotedtext{\hlcyan{I might use it, but I feel there are sources that I'm already comfortable with [...] I Google it. It's more accessible. I do stick to very traditional sites where I can trust the answers.}} -[P13]

While participants expressed inhibitions towards adopting ChatGPT as an \hlcyan{integral part of their CS academic workflow}, they seemed hopeful about its future positive impact on education. A participant referred to it as a \textit{revolution in education} if it's used rightly. ChatGPT is being seen as the future `Google search'. Various participants said that this change is inevitable and we should accept it with an open mind. 

\quotedtext{\hlcyan{You can't go about your education without using Google. You need it for everything. It's incorporated into the system now. I feel the same. That's what will happen with ChatGPT in the future.}} -[P9] 

Participants suggested enhancing ChatGPT and related services for improved user experience. Multi-modality input was a common theme. They emphasized the necessity of training for efficient prompting and optimal use. A confidence score feature to authenticate the validity of answers was proposed. Effective multilingual capabilities for inclusivity were also suggested. \hlcyan{Some participants mentioned that domain-specific versions of ChatGPT for various CS courses can help offer insightful and reliable information in specific fields}.

\quotedtext{\hlcyan{Maybe it can start providing some tutorials on it soon. Is it possible? If it is possible, then it's really good. Like when we just open ChatGPT, it can show a few options like learn this, learn that I will make you learn this.}} -[P2]

==> files/061-acknowledgements.tex <==
We are grateful to anonymous reviewers for their feedback, which improved the overall quality of the article. We thank Shamik Sinha, Palak Bhardwaj, Rayyan Hussain, Kashvi Panvanda, Sidhartha Garg, Shagun Yadav and Sourav Goyal for their assistance in the development of questionnaires, as well as their involvement in conducting selected interviews.
